Spatial Attention as an Interface for Image Captioning Models

The internal workings of modern deep learning models stay often unclear to an external observer, although spatial attention mechanisms are involved. The idea of this work is to translate these spatial attentions into natural language to provide a simpler access to the model's function. Thus, I took a neural image captioning model and measured the reactions to external modification in its spatial attention for three different interface methods: a fixation over the whole generation process, a fixation for the first time-steps and an addition to the generator's attention. The experimental results for bounding box based spatial attention vectors have shown that the captioning model reacts to method dependent changes in up to 52.65% and includes in 9.00% of the cases object categories, which were otherwise unmentioned. Afterwards, I established such a link to a hierarchical co-attention network for visual question answering by extraction of its word, phrase and question level spatial attentions. Here, generated captions for the word level included details of the question-answer pairs in up to 55.20% of the cases. This work indicates that spatial attention seen as an external interface for image caption generators is an useful method to access visual functions in natural language.

==> Chapters/Chapter1_vqa.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{An example}

% image id 9
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/dishes}
	\decoRule
	\caption[An Electron]{A sample image for visual question answering}
	\label{fig:sample}
\end{figure}

\subsection{Training captions}
\begin{enumerate}
	\item[(1)] 	Closeup of bins of food that include broccoli and bread.
	\item[(2)] 	A meal is presented in brightly colored plastic trays.
	\item[(3)] 	there are containers filled with different kinds of foods
	\item[(4)] 	Colorful dishes holding meat, vegetables, fruit, and bread.
	\item[(5)] 	A bunch of trays that have different food.
\end{enumerate}

Assumption: The pre-trained caption generation network is capable to produce the captions given for the image.

% question ids [90, 91, 92]
\subsection{Questions and answers}
\begin{enumerate}
	\item[(A)] \textbf{What color are the dishes?} Ground-truth answer: pink and yellow	
	\item[(B)] \textbf{How many cookies can be seen?} Ground-truth answer: 2
	\item[(C)] \textbf{What is the green stuff?} Ground-truth answer: broccoli
\end{enumerate}

\subsection{Case: Question (A) and Caption (4)}

The co-attention network is presented the question (A) 
\begin{verbatim}
	What color are the dishes?
\end{verbatim}

Given the word \textit{dishes} in the question, the co-attention network computes a soft attention for the boxes in the image. Given the image soft attention, the caption network produces a sentence similar to (4).

\begin{verbatim}
	Colorful dishes holding meat, vegetables, fruit, and bread.
\end{verbatim}

Since the captions do not provide the answer, the network learns the answer from the training answers.

\begin{verbatim}
pink and yellow
\end{verbatim}

 In the best case, the co-attention network learns to correlate \textbf{colorful} with \textbf{pink and yellow}.

\subsection{Case: Question (B) and Caption (5)}

The co-attention network is presented the question (B) 
\begin{verbatim}
How many cookies can be seen?
\end{verbatim}

Given the word \textit{How many} in the question, the co-attention network computes a soft attention for the individual items in the image. Given the image soft attention, the caption network produces a sentence similar to (1).

\begin{verbatim}
	A bunch of trays that have different food.
\end{verbatim}

Since the captions do not provide the answer, the network learns the answer from the training answers. 

\begin{verbatim}
2
\end{verbatim}

In the best case, the co-attention network learns the soft-attention for the cookies (on the right side) from the answers and the captioning network has seen cookies on other images in the training set to produce appropriate captions later on.

\subsection{Case: Question (C) and Caption (1)}

The co-attention network is presented the question (A) 
\begin{verbatim}
What is the green stuff?
\end{verbatim}

Given the word \textit{green} in the question, the co-attention network computes a soft attention for the broccoli in the image. Given the image soft attention, the caption network produces a sentence similar to (1).

\begin{verbatim}
Closeup of bins of food that include broccoli and bread.
\end{verbatim}

Since the captions does provide the answer, the network selects the answer directly from the caption. 

\begin{verbatim}
broccoli
\end{verbatim}

Here the caption generation network is providing the world-knowledge to answer the question.

